An Efficient Approach to Generate Safe Drivable Space by LiDAR-Camera-HDmap Fusion

In this paper, we propose an accurate and robust perception module for Autonomous Vehicles (AVs) for drivable space extraction. Perception is crucial in autonomous driving, where many deep learning-based methods, while accurate on benchmark datasets, fail to generalize effectively, especially in diverse and unpredictable environments. Our work introduces a robust easy-to-generalize perception module that leverages LiDAR, camera, and HD map data fusion to deliver a safe and reliable drivable space in all weather conditions. We present an adaptive ground removal and curb detection method integrated with HD map data for enhanced obstacle detection reliability. Additionally, we propose an adaptive DBSCAN clustering algorithm optimized for precipitation noise, and a cost-effective LiDAR-camera frustum association that is resilient to calibration discrepancies. Our comprehensive drivable space representation incorporates all perception data, ensuring compatibility with vehicle dimensions and road regulations. This approach not only improves generalization and efficiency, but also significantly enhances safety in autonomous vehicle operations. Our approach is tested on a real dataset and its reliability is verified during the daily (including harsh snowy weather) operation of our autonomous shuttle, WATonoBus

==> 2-methods-backup.tex <==
\section{Methods}
\label{sec:methods}
Our method involves a series of precise steps to determine the drivable space for autonomous vehicles. Initially, LiDAR and camera data undergo a sequence of pre-processing; we crop the point cloud to the region of interest (ROI) defined by HD map data, including curbs and sidewalks. Next, we perform an adaptive ground removal process to isolate points above the ground level, focusing on the right curb. Following this, we apply clustering techniques to organize the remaining points. Concurrently, we process images captured from six cameras using the YOLO algorithm to identify and label various objects, which are then fused with the previously clustered point data. Additionally, we integrate the centerline data from the HD map to enhance the accuracy of our spatial analysis. Finally, we utilize the data from obstacles, the right curb, and the centerline to precisely delineate the final drivable space.



\subsection{Inputs Pre-processing}
\subsubsection{Point Cloud Pre-processing, Consistent Concatenation}
To make sure the autonomous vehicle can achieve a 360\textdegree \ perception coverage, one vehicle can be equipped with $N_L$ LiDAR sensors. Let one sweep of point cloud of LiDAR sensor k be $\mathbb{P}_k=\{ P_k^1, P_k^2, \cdots, P_k^{N_k}\}$, where each point $P_k^i = \{x, y, z, \text{intensity}, \text{ring}, \text{timestamp}\}$ contains the 3D position, reflection intensity, the ring index of its beam, and timestamp of receiving this point. The point clouds from different sensors are first transformed into a fixed coordinate system $G$, then they are concatenated into an overall point cloud $\mathbb{P}$. 
For a typical mechanical LiDAR, it takes about 100ms to get a scan of point cloud, meaning the position measurement may not be accurate due to the ego vehicle motion. To eliminate this, the timestamp of each point is used to find the transformation to the current time based on the odometry data.
\subsubsection{HD Map Utilization}
The HD map stores the positions of the left and right road boundaries, i.e. curbs. The localization information is used to transform the left and right curb positions from the global map frame into the local vehicle frame. It's worth noting that even though we call it HD map here, the required precision is not necessarily centimeter level, it mainly provides the coarse road boundaries information for the following tasks.

%As demonstrated in (TODO, add the case that recent construction modified the right curb position), the proposed method still performs properly even the HD map is not accurate.
\subsubsection{Camera-LiDAR Pre-processing, Calibration}
This part includes the camera intrinsic and extrinsic calibration where one checkerboard is needed. The camera intrinsic calibration is based on \cite{888718}. The extrinsic calibration is achieved by minimizing the projection error from the point cloud to the image pixel.
% The code is available here\footnote{\url {https://github.com/NingMingHao/LiDARCameraCalibration}}.

\subsection{Adaptive Grid Ground Removal and Curb Detection}
Based on the coarse road boundaries from the HD map, the overall point cloud is divided into multiple grids, and plane estimation is performed for each grid. Then the non-ground points near the road boundaries will be selected as candidate curb points, which will be used for the curb detection. The algorithm is summarized in Algorithm \ref{algorithm:adaptive_grid_ground_removal}.
For the region closest to the vehicle, it uses the height of the LiDAR sensor as the initial plane model, then iteratively improves the plane fitting. This estimation serves as the initial value for ground estimation in other regions. One of the key strengths of the adaptive grid ground removal algorithm is its ability to adjust road surface fitting thresholds based on the distance from the vehicle. More stringent fitting thresholds are set for areas closer to the vehicle, which ensures small objects can be detected within safety distance. 
%TODO: add two figures, one geese detection (with curb detection in normal case), and another figure shows the case that snow pile covers the right curb.
% \begin{comment}
\begin{algorithm}
    \label{algorithm:adaptive_grid_ground_removal}
    \caption{Ground Removal and Curb Detection}
    \SetKwFunction{isOddNumber}{isOddNumber}
    \SetKwInOut{KwIn}{Input}
    \SetKwInOut{KwOut}{Output}
    \SetKwInOut{KwInit}{Initialize}
    \SetKwInOut{KwRet}{Return}

    \KwIn{A list of points $\mathbb{P} = \{P_1, \cdots, P_N\}$, a list of grids $\mathbb{G} = \{G_1, \cdots, G_M\}$ sorted by the distance to the vehicle, where $N$ denotes the number of points and $M$ denotes the number of grids.}
    \KwOut{A list of boolean values denoting if it's an obstacle point $\mathbb{O} = \{O_1, \cdots, O_N\}$,  a list of estimated ground plane models $\mathbb{F} = \{z=f_1(x,y), \cdots, z=f_M(x,y)\}$, a second-order function $y=f_C(x)$ denoting the curb position.}
    \KwInit{Set height of the LiDAR $h_L$, height of curb $h_C$, set threshold parameters $\{T_1, \cdots, T_M\}$, set the maximum number of iterations $N_{\max}$ and convergence threshold $\epsilon$.
    Set initial nearby ground fit $f_0=-h_L$.}
    Part 1: Adaptive Grid based Ground Removal
    
    \setcounter{AlgoLine}{0}
    \SetNlSty{textbf}{1-}{}
    \For{$i=1$ \KwTo $M$}
    {
        Find points $\mathbb{P}_i$ in grid $G_i$, set $f_i^1=f_{i-1}$.

        \For{$j = 1$ \KwTo $N_{\max}$}{
            Find inliers $\mathbb{P}_{In} = \{P_k | (|z_k - f_i^{j}(x_k,y_k)| \leq T_i), P_k \in \mathbb{P}_i\}$
             
            Fit a new model $f_i^{j+1}$ by minimizing the estimation error of the inliers $\mathbb{P}_{In}$. $f_i^{j+1} = \min_{f} \sum_{P_k \in \mathbb{P}_{In}} (z_k - f(x_k, y_k))^2$

            \If{$\|f_i^{j} - f_i^{j+1}\|<\epsilon$}{
            \textbf{converge and early stop}
            }
        }
        Set the boolean value of inliers as \texttt{False} and outliers as \texttt{True} in $\mathbb{O}$, save $f_i$ into $\mathbb{F}$.
    }
    \setcounter{AlgoLine}{1}
    \SetNlSty{textbf}{}{}
    Part 2: Curb Detection
    
    \setcounter{AlgoLine}{0}
    \SetNlSty{textbf}{2-}{}
    Select the candidate curb points $\mathbb{P}_C$ near the coarse road boundaries from the obstacle points whose distance to the ground plane is less than $h_C$ and its corresponding grid covers the road boundary.
    
    Periodically select top K innermost points to the road from $\mathbb{P}_C$ according to $x$, and add them to $\mathbb{P}_C^K$.
    
    Perform robust polynomial fitting to $\mathbb{P}_C^K$ and get the curb model $y=f_C(x)$.

    \setcounter{AlgoLine}{2}
    \SetNlSty{textbf}{}{}
    Part 3: Tune $\mathbb{O}$ based on curb model $f_C$
    
    \setcounter{AlgoLine}{0}
    \SetNlSty{textbf}{3-}{}
    \For{\texttt{each} $p_i$ \textbf{in} $\mathbb{P}_C$}
    {
        Determine whether the point $p_i$ lies within the boundaries of the road by comparing its $y$-coordinate to the value given by the curb model function $f_C$. 

        If $p_i$ is on the road, then assign the corresponding index in the $\mathbb{O}$ a value of \texttt{True}.
        
        If $p_i$ is within the sidewalk region, then assign the corresponding index in the $\mathbb{O}$ a value of \texttt{False}.
    }
\end{algorithm}

\subsection{Camera based Perception}
Cameras provide rich color and texture information, while they lack depth information. So, the images are used for 2D detection, i.e., detecting features on the image plane. Camera 2D detection has been well studied recently in the deep learning field. Compared to 3D detection, it has more public datasets as it's much easier to label 2D features on the image plane than 3D coordinate which may need stereo vision or other high-density range sensors to provide depth information. Also, the single camera based 3D detection doesn't generalize as good as 2D detection as it's difficult to estimate depth information for cameras with different configurations. Two state-of-the-art neural networks are optimized and then used in this paper to provide 2D object detection and 2D lane detection.
\subsubsection{YOLOv8}
YOLOv8 \cite{yolov8_ultralytics} is one of YOLO (You Only Look Once) series of real-time object detectors. It employs state-of-the-art backbone and neck architectures, making it achieving high accuracy with high inference speed. A customized dataset for outdoor autonomous driving usage has been created by selecting interesting objects from public datasets including COCO (Common Objects in Context) \cite{lin2015microsoft}, Argoverse \cite{Argoverse} and nuScenes \cite{nuscenes}. 
% The summary of the customized dataset is shown in Fig. ????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????\ref{fig:dataset-instances}
% \begin{figure}[htb]
%     \centering
%     \includegraphics[width=0.3\textwidth]{figs/DatasetInstances.jpg}
%     \caption{Summary of Customized Dataset for YOLOv8}
%     \label{fig:dataset-instances}
% \end{figure}
Then the YOLOv8 is trained on 90\% of the dataset, and evaluated on the rest 10\% of the dataset, and mAP50 of 0.708 has been achieved. Finally, the trained model is converted to TensorRT model for best inference speed. 
% The code is available here\footnote{\url {https://github.com/NingMingHao/Yolov8TensorrtRos}}.
\subsubsection{UFLDv2}
UFLDv2 \cite{qin2022ultrav2} treats the lane detection task as an anchor-driven ordinal classification problem using global features, it can achieve both remarkable speed and accuracy. The output of the UFLDv2 is a set of lane marker points in the image plane, to obtain the lane marker position in the real world, the ground plane models $\mathbb{F}$ from the adaptive ground removal method are used to provide the road geometry information, then the 3D positions of the lane markers can be inferred using the inverse camera projection under the assumption that the markers are located on the estimated ground planes.
% The code is available here\footnote{\url {https://github.com/NingMingHao/LaneDetectionAndPostProcess}}.

\subsection{Adaptive Clustering for All Weather Conditions}
%TODO: add a figure of noisy point cloud with camera view.
%TODO: Add a figure showing the LiDAR Scanning pattern and the voxel downsample.
Falling rain and snow can introduce amounts of noisy reflections to the LiDAR sensors.  Failing to de-noise point cloud may lead to false detection, and even trigger the emergency stop. Although clustering methods like DBSCAN \cite{DBSCAN} can somehow ease this by setting a smaller clustering distance threshold $\epsilon$ or a larger minimum number of points required to form a core region $\text{minPts}$. However, this will inevitably remove points from actual objects, and also introduce over-segmentation issue, where the points from the same object will be clustered into several groups. We improve this by proposing an adaptive DBSCAN clustering method that uses the LiDAR scanning pattern to adaptively adjust the $\epsilon$ and $\text{minPts}$.

Assume we have a plane object with height $h$ and width $\omega$ facing the LiDAR at a distance of $s$, whose horizontal scanning resolution is $\Delta \varphi$ and vertical resolution is $\Delta \alpha$. For a more general case, the point cloud is usually first downsampled with a voxel size $\Delta d$ to reduce the processing time. Then the number of scan lines $N_{s}$ and the number of points in each line $N_{pl}$ falling to the plane object will be,
\begin{equation}
N_{s} = floor(\frac{h}{\max(s\Delta \alpha, \Delta d) }) 
\end{equation}
\begin{equation}
N_{pl} = floor(\frac{w}{\max(s\Delta \varphi, \Delta d) }) 
\end{equation}

Here, we propose an Adaptive-DBSCAN that will dynamically adjust the $\epsilon$ and $\text{minPts}$ based on the LiDAR scanning pattern. In this method, the $\epsilon$ is adjusted to have a constant $N_{pl}$,
\begin{equation}
    N_{pl} = floor(\omega_{\min} / \Delta d) \ 
\end{equation}
where $\omega_{\min}$ is the minimum width of the objects in the environment.
Then the clustering distance threshold will be,
\begin{equation}
    \epsilon (s)= \max(\omega_{\min},\hspace{2.5pt}N_{pl} \Delta \varphi s)
\end{equation}
The number of scanning lines will be,
\begin{equation}
    N_{s} (s) = \max(1,\hspace{2.5pt}floor(\frac{h_{\min}}{\max(s\Delta \alpha,\hspace{2.5pt}\Delta d) }) )
\end{equation}
where $h_{\min}$ is the minimum height of the objects in the environment, and the $\text{minPts} = N_{s}N_{pl}$.

\subsection{Robust LiDAR Camera Fusion}
This part aims to fuse the object clustering results from the LiDAR and the 2D object detection results from the cameras to obtain clusters with semantic information. To achieve this, an association cost is calculated for each cluster and each 2D bounding box, and the Hungarian algorithm \cite{hungmatch} is used to find the best associations. The key to improving the LiDAR-camera fusion performance is the way to calculate the association cost. The 2D association cost based on the intersection over union (IOU) of the camera bounding box and the projected cluster points bounding box is a common choice due to its simplicity. However, it fails in handling distant objects where the bounding box is small and the intersection region could be zero due to imperfect calibration or object motion. We fix this issue by introducing the 3D information into the association cost.

\begin{figure}[tb]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/camera_projection.pdf}
    \caption{Camera Projection}
    \label{fig:camera-projection}
\end{figure}

A depth and its uncertainty estimation method using the semantic 2D bounding box is proposed. Considering a common camera placement scheme as shown in Fig. \ref{fig:camera-projection}, where there is a pitch angle $\theta$ between the camera coordinate plane $X_cOZ_c$ and the world coordinate plane $X_wOZ_w$ parallel to the ground surface. The projection of a point $P_w=(x_w,y_w,z_w)$ in the world coordinate to the pixel coordinate $p_p=(x_p, y_p)$ can be expressed as 
\begin{equation}
\begin{split}
    s \begin{bmatrix} x_p \\ y_p \\ 1 \end{bmatrix} &= K R_\theta \begin{bmatrix} x_w \\ y_w \\ z_w \end{bmatrix} \\
    &= \begin{bmatrix} f_x & 0 & c_x \\ 0 & f_y & c_y \\ 0 & 0 & 1 \end{bmatrix} \begin{bmatrix} 1 & 0 & 0 \\ 0 & \cos{\theta} & -\sin{\theta} \\ 0 & \sin{\theta} & \cos{\theta} \end{bmatrix} \begin{bmatrix} x_w \\ y_w \\ z_w \end{bmatrix}
    % &= \begin{bmatrix} f_x & c_x \sin{\theta} & c_x \cos{\theta} \\ 0 & c_y \sin{\theta} + f_y \cos{\theta} & c_y \cos{\theta} - f_y \sin{\theta} \\ 0 & \sin{\theta} & \cos{\theta} \end{bmatrix} \begin{bmatrix} x_w \\ y_w \\ z_w \end{bmatrix}
\end{split}
\end{equation}

Based on this projection matrix, for an object having a fixed distance $z_w$, we have:
\begin{subequations}
\begin{equation}
  s = y_w \sin{\theta} + z_w \cos{\theta} 
\end{equation}    
\begin{equation}
  s \Delta x_p = f_x \Delta x_w
\end{equation}
\begin{equation}
  s \Delta y_p = ( (c_y-y_p) \sin{\theta} + f_y \cos{\theta} ) \Delta y_w
\end{equation}
\end{subequations}

Replace the $\Delta x_w$ and $\Delta y_w$ to $W_w$ and $H_w$ denoting the width and height of the object in the world coordinate, and replace the $\Delta x_p$ and $\Delta y_p$ to $W_p$ and $H_p$ denoting the width and height of the 2D image bounding box of the object. The $y_w$ and $y_p$ will be the $y$-coordinate of the center of the object and bounding box, respectively. For an object standing on the ground, $y_w=H_w^{cam} - H_w/2$, where $H_w^{cam}$ denotes the height of the camera relative to the ground plane. So to calculate the final distance $z_w$ and its uncertainty $\sigma_z^2$, we need to calculate the depth estimation based on width and the height prior. Estimation based on width:
\begin{subequations}
    \begin{equation*}
        z_{w}^{\omega} = \frac{f_x W_w}{W_p \cos{\theta}} - y_w \tan{\theta}
    \end{equation*}
    \begin{equation*}
        \sigma_{z}^{\omega^2} = \frac{W_p^4 \sigma_{y_w}^2 \sin^2{\theta} + W_p^2 f_x^2 \sigma_{W_w}^2 + W_w^2 f_x^2 \sigma_{W_p}^2}{W_p^4 \cos^2{\theta}}
    \end{equation*}
    \begin{equation*}
        \sigma_{y}^{\omega^2} = \sigma_{H_w^{cam}}^2 + {\sigma_{H_w}^2}/{4}
    \end{equation*}
\end{subequations}

and the estimation based on height:
\begin{subequations}
    \begin{equation*}
        z_{w}^{h} = \frac{ ( (c_y-y_p) \sin{\theta} + f_y \cos{\theta} )H_w}{H_p \cos{\theta}} - y_w \tan{\theta}
    \end{equation*}
    \begin{align*}
        \sigma_{z}^{\omega^2} & =  \frac{1}{H_{p}^{4} \cos^{2}{\theta}}  \left[ H_{p}^{4} \sigma_{{H_{w}^{cam}}}^{2} \sin^{2}{\theta} \right. \\
    & + \frac{H_{p}^{2} \sigma_{H_w}^{2} \left(H_{p} \sin{\theta} + 2 f_{y} \cos{\theta} + 2 \left(c_{y} - y_{p}\right) \sin{\theta}\right)^{2}}{4} \\
    & + H_{w}^{2} \sigma_{H_p}^{2} \left(f_{y} \cos{\theta} + \left(c_{y} - y_{p}\right) \sin{\theta}^{2} \right]
    \end{align*}
\end{subequations}

Finally, the measurements are averaged based on the variances:
\begin{subequations}
\begin{equation}
  z_w = \frac{z_{w}^{h}\sigma_{z}^{\omega^2} + z_{w}^{\omega} \sigma_{z}^{h^2}}{\sigma_{z}^{\omega^2} + \sigma_{z}^{h^2}}
\end{equation}    
\begin{equation}
  \sigma_{z}^2 = \frac{\sigma_{z}^{h^2} \sigma_{z}^{\omega^2}}{\sigma_{z}^{\omega^2} + \sigma_{z}^{h^2}}
\end{equation}
\end{subequations}

This estimated depth information will be used as part of the association cost defined as,
\begin{equation}
    \pi_{i,j} = \delta(1-\text{IOU}_{i,j}) + (1-\delta)\Delta(\rho_{w}^{cam}, \rho_{w}^{Li})
\end{equation}
where, $\text{IOU}_{i,j}$ is calculated between the LiDAR projected bounding box, and the camera's, $\delta$ is the importance weight, $\Delta()$ takes the mahalanobis distance between the object position estimate from camera, $\rho_{w}^{cam}$, and from LiDAR, $\rho_{w}^{Li}$, and $\pi_{i,j}$ forms the Hungarian matrix $\Pi_{Li}^{cam}$, and can be solved with Hungarian matching algorithm in \cite{hungmatch}.

\subsection{Drivable Space Detection}
In constructing a comprehensive representation of drivable space, our method integrates the above lane and curb detection, objects with class information, and the HD map data. It accounts for ego vehicle dimensions and dynamics, object class information and road regulations, thereby facilitating a safe and lawful autonomous driving behavior.

Firstly, detected objects are projected onto the HD map to get the identification of objects positioned within the ego lane, the opposing lane, on sidewalks, or at crosswalks.
Subsequently, a binary occupancy map is constructed utilizing the positional data of objects, lanes, and curbs. This map shows occupied regions, which are further adjusted based on object class, as well as the dimensions and velocity of the ego vehicle to define a safety envelope for navigation.
For lateral expansion, the clearance required for each object is computed as the sum of a predefined distance relative to the object's class and half the width of the ego vehicle. The longitudinal expansion incorporates an additional term representing the minimum braking distance, calculated as $v^2/(2a)$, where $v$ is the velocity of the ego vehicle and $a$ is the deceleration rate.
Vulnerable road users, such as pedestrians and cyclists, are allocated an increased clearance for safety reasons. A special case is applied to pedestrians on crosswalks, the lateral expansion is adjusted to span the entire road width so the ego vehicle will stop until the object walks off the crosswalk.

The refined binary occupancy grid is processed and simplified into a series of boundary points, which is the drivable space boundary. This is achieved by building a connection tree starting from the ego position that grows along the longitudinal direction and connects the safety region segments. This tree is searched and gives the final left-side and right-side drivable space boundary.
